Gradient-based Novelty Detection Boosted by Self-supervised Binary Classification

Novelty detection aims to automatically identify out-of-distribution (OOD) data, without any prior knowledge of them. It is a critical step in data monitoring, behavior analysis and other applications, helping enable continual learning in the field. Conventional methods of OOD detection perform multi-variate analysis on an ensemble of data or features, and usually resort to the supervision with OOD data to improve the accuracy. In reality, such supervision is impractical as one cannot anticipate the anomalous data. In this paper, we propose a novel, self-supervised approach that does not rely on any pre-defined OOD data: (1) The new method evaluates the Mahalanobis distance of the gradients between the in-distribution and OOD data. (2) It is assisted by a self-supervised binary classifier to guide the label selection to generate the gradients, and maximize the Mahalanobis distance. In the evaluation with multiple datasets, such as CIFAR-10, CIFAR-100, SVHN and TinyImageNet, the proposed approach consistently outperforms state-of-the-art supervised and unsupervised methods in the area under the receiver operating characteristic (AUROC) and area under the precision-recall curve (AUPR) metrics. We further demonstrate that this detector is able to accurately learn one OOD class in continual learning.

==> bib_bk.tex <==
@inproceedings{kwon2020backpropagated,
  title={Backpropagated Gradient Representations for Anomaly Detection},
  author={Kwon, Gukyeong and Prabhushankar, Mohit and Temel, Dogancan and AlRegib, Ghassan},
  booktitle={European Conference on Computer Vision},
  pages={},
  year={2020},
  organization={Springer}
}

@article{hendrycks2016baseline,
  title={A baseline for detecting misclassified and out-of-distribution examples in neural networks},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1610.02136},
  year={2016}
}


@inproceedings{lee2020gradients,
  title={Gradients as a Measure of Uncertainty in Neural Networks},
  author={Lee, Jinsol and AlRegib, Ghassan},
  booktitle={2020 IEEE International Conference on Image Processing (ICIP)},
  pages={2416--2420},
  year={2020},
  organization={IEEE}
}

@inproceedings{abati2019latent,
  title={Latent space autoregression for novelty detection},
  author={Abati, Davide and Porrello, Angelo and Calderara, Simone and Cucchiara, Rita},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={481--490},
  year={2019}
}


@article{lee2018simple,
  title={A simple unified framework for detecting out-of-distribution samples and adversarial attacks},
  author={Lee, Kimin and Lee, Kibok and Lee, Honglak and Shin, Jinwoo},
  journal={arXiv preprint arXiv:1807.03888},
  year={2018}
}


@article{liang2017enhancing,
  title={Enhancing the reliability of out-of-distribution image detection in neural networks},
  author={Liang, Shiyu and Li, Yixuan and Srikant, Rayadurgam},
  journal={arXiv preprint arXiv:1706.02690},
  year={2017}
}

@article{sehwag2021ssd,
  title={Ssd: A unified framework for self-supervised outlier detection},
  author={Sehwag, Vikash and Chiang, Mung and Mittal, Prateek},
  journal={arXiv preprint arXiv:2103.12051},
  year={2021}
}


@article{goodfellow2014generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.2661},
  year={2014}
}


@inproceedings{kwon2020novelty,
  title={Novelty detection through model-based characterization of neural networks},
  author={Kwon, Gukyeong and Prabhushankar, Mohit and Temel, Dogancan and AlRegib, Ghassan},
  booktitle={2020 IEEE International Conference on Image Processing (ICIP)},
  pages={3179--3183},
  year={2020},
  organization={IEEE}
}


@inproceedings{sakurada2014anomaly,
  title={Anomaly detection using autoencoders with nonlinear dimensionality reduction},
  author={Sakurada, Mayu and Yairi, Takehisa},
  booktitle={Proceedings of the MLSDA 2014 2nd Workshop on Machine Learning for Sensory Data Analysis},
  pages={4--11},
  year={2014}
}


@article{paszke2017automatic,
  title={Automatic differentiation in pytorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  year={2017}
}


@article{cifar,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Citeseer}
}


@article{netzer2011reading,
  title={Reading digits in natural images with unsupervised feature learning},
  author={Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y},
  year={2011}
}




@inproceedings{resnet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{ILSVRC15,
Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
Title = {{ImageNet Large Scale Visual Recognition Challenge}},
Year = {2015},
journal   = {International Journal of Computer Vision (IJCV)},
doi = {10.1007/s11263-015-0816-y},
volume={115},
number={3},
pages={211-252}
}


@misc{yu2016lsun,
      title={LSUN: Construction of a Large-scale Image Dataset using Deep Learning with Humans in the Loop}, 
      author={Fisher Yu and Ari Seff and Yinda Zhang and Shuran Song and Thomas Funkhouser and Jianxiong Xiao},
      year={2016},
      eprint={1506.03365},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}



@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{zhou2017anomaly,
  title={Anomaly detection with robust deep autoencoders},
  author={Zhou, Chong and Paffenroth, Randy C},
  booktitle={Proceedings of the 23rd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={665--674},
  year={2017}
}


@inproceedings{chen2017outlier,
  title={Outlier detection with autoencoder ensembles},
  author={Chen, Jinghui and Sathe, Saket and Aggarwal, Charu and Turaga, Deepak},
  booktitle={Proceedings of the 2017 SIAM international conference on data mining},
  pages={90--98},
  year={2017},
  organization={SIAM}
}



@inproceedings{hawkins2002outlier,
  title={Outlier detection using replicator neural networks},
  author={Hawkins, Simon and He, Hongxing and Williams, Graham and Baxter, Rohan},
  booktitle={International Conference on Data Warehousing and Knowledge Discovery},
  pages={170--180},
  year={2002},
  organization={Springer}
}

@inproceedings{du2021enas,
  title={Evolutionary NAS in Light of Model Stability for Accurate Continual Learning},
  author={ Du, Xiaocong and Li, Zheng and Sun, Jingbo and Liu, Frank and Cao, Yu},
  booktitle={2021 International Joint Conference on Neural Networks (IJCNN)},
  pages={----},
  year={2021},
  organization={IEEE}
}


@inproceedings{du2020noise,
  title={Noise-based selection of robust inherited model for accurate continual learning},
  author={Du, Xiaocong and Li, Zheng and Seo, Jae-sun and Liu, Frank and Cao, Yu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={244--245},
  year={2020}
}

==> response.tex <==
\section{Response to Reviewer 1}

We sincerely thank you for your time and efforts. Regarding the computational complexity, we conduct several optimizations. For example, we only collect the gradients from the last layer of the feature extractor to perform the novelty detection and still achieve high performance. We also choose a simple structure for the binary classifier (3 Convolutional layers + Sigmoid), which only requires a few epochs to train. Overall the computation of the proposed method is efficient. 

%In addition, we test various methods to recufor the mean and precision matrix estimation, we test various methods to reduce the number of samples needed in the calculation, such as that based on importance sampling to help select the samples to best represent the corresponding gradient distribution. With fewer samples in gradient calculation, the computation complexity will be reduced in proportion.

\section{Response to Reviewer 2}

Thank you for your review and comments. We will continue to delve into the theoretical side of our proposed approach, such as the stability of the iteration between the Mahalanobis distance-based detector and the binary classifier.

\section{Response to Reviewer 3}
We sincerely thank you for your time and efforts. Please find the response for each question.


\textbf{Why using Mahalanobis distance of gradients rather than just gradients?} \\
During the early stage of the research, we tried to use the gradients themselves to detect the OOD because intuitively, the OOD should generate a large gradient. However we found that this method was not effective when the OOD are very similar to the IDD samples. For example, if a model is trained to recognize the 'automobile' class of CIFAR-10, then it will give relatively high confidence (i.e., low gradients) to the 'truck' class, which has similar features of the 'automobile'. A similar trend was also observed between 'bird' and 'airplane'. Therefore we choose a more precise measure metric, the Mahalanobis distance, which works much better than the gradients themselves.

\textbf{Estimate the precision matrix as the same over all the training classes} 

We are inspired by the paper (Lee et al. 2018), which is based on the linear discriminant analysis that assumes all classes share the same precision matrix.

\textbf{In Eq. (4), define label y for each sample instead of a batch?}


This label is only estimated once and then fixed, and the upcoming OODs will use this label to do the backpropagation for the gradients. The purpose of Eq. (4) is to find the least likely class that the OODs belong to, such that the gradients for the OODs can be maximized. To best estimate this label, a batch of OODs is preferred.

\textbf{In Fig. 5-(c), Why use 50\% instead of 100\%?}

This ablation study is to check how the training performance of the binary classifier is affected by different percentages of the novelty detector's IDD/OOD prediction. If we use 100\%, it means we create a training dataset assuming the novelty detector is 100\% accurate in the IDD/OOD prediction. In reality, there will be some error in the prediction and therefore, the training dataset will be mislabeled. So we choose 50\% or less in order to filter out those mislabeled data for the best training performance.

We  appreciate your comments that point out other writing issues in our paper. We will fix them in the final version. 




\section{Response to Reviewer 4}
We sincerely thank you for your time and efforts. Please find the response for each question.


\textbf{Justification on why the refinement step is able to overcome initial misclassifications}

The initial mis-classification is due to the use of the predicted label for both IDD and OOD, which generates the minimum gradients and the Mahalanobis distance. For OOD, we want its Mahalanobis distance to be large and thus, we carefully select another label that maximizes the loss for a larger Mahalanobis distance. As shown in Fig. 3, the distribution of the Mahalanobis score is shifted from the blue region to the green region, which in turn eases the search of an appropriate threshold to separate the red (IDD) and green (OOD).

\textbf{The experimental configures all run with batches of strictly IDD or ODD data}

The batch mode is only used in the training and inference of the binary classifier, which effectively improves its accuracy. On the other side, our primary novelty detector, which is based on the Mahalanobis distance, does not require the batch mode. It is able to work for each single input. In practice, we can employ our primary novelty detector to make the initial IDD/OOD prediction one by one, and then collect the samples into the corresponding IDD or OOD batch. Once a batch is ready, it will be sent to the binary classifier for the downstream work.

Such a batch-mode operation of the binary classifier is also used in the generative adversarial network (GAN) (Goodfellow
et al. 2014) that helps distinguish very similar images. 


\textbf{Numerical reporting lacks sufficient sig figs or any confidence intervals}


We agree with the reviewer's suggestion to conduct multiple runs and report standard deviations. For CIFAR-100 vs. CIFAR-10, which is the challenging datasets to separate, we conduct 10 runs and the average AUROC/AUPR are 88.61/85.45 and their standard deviation are 1.063/1.114. We will further conduct the experiments on other benchmarks and present the results in the final version. 





\newpage



